Deep Neural Network Benchmarks for Selective Classification

With the increasing deployment of machine learning models in many socially sensitive tasks, there is a growing demand for reliable and trustworthy predictions. One way to accomplish these requirements is to allow a model to abstain from making a prediction when there is a high risk of making an error. This requires adding a selection mechanism to the model, which selects those examples for which the model will provide a prediction. The selective classification framework aims to design a mechanism that balances the fraction of rejected predictions (i.e., the proportion of examples for which the model does not make a prediction) versus the improvement in predictive performance on the selected predictions. Multiple selective classification frameworks exist, most of which rely on deep neural network architectures. However, the empirical evaluation of the existing approaches is still limited to partial comparisons among methods and settings, providing practitioners with little insight into their relative merits. We fill this gap by benchmarking 18 baselines on a diverse set of 44 datasets that includes both image and tabular data. Moreover, there is a mix of binary and multiclass tasks. We evaluate these approaches using several criteria, including selective error rate, empirical coverage, distribution of rejected instance's classes, and performance on out-of-distribution instances. The results indicate that there is not a single clear winner among the surveyed baselines, and the best method depends on the users' objectives.

==> tex_files/best_tables.tex <==
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \DG{}, divided by architectures.}
\label{tab:best_perf_dg}
\begin{tabular}{ccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} &    $o$ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &             SGD &              $1e-03$ &               $1e-04$ &      \texttt{False} &            $.92$ &    \texttt{False} &  $1.0$ &                $1$ &             $320$ &               $.30$ &                &                  $2.67$ &               & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.20$ &                 &                  $1.33$ &              $.45$ &                                                            \\
    \texttt{covtype} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &  $4.2$ &                $2$ &             $512$ &               $.15$ &               $.20$ &                  $1.67$ &              $.10$ &                                                            \\
\texttt{electricity} &            Adam &              $1e-05$ &               $1e-03$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &             $192$ &               $.05$ &                 &                  $1.00$ &              $.50$ &                                                            \\
        \texttt{eye} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
      \texttt{heloc} &           AdamW &              $1e-05$ &               $1e-05$ &       \texttt{True} &              &       &  $1.8$ &                $3$ &             $384$ &               $.25$ &               $.10$ &                  $1.33$ &              $.45$ &                                                            \\
      \texttt{higgs} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
      \texttt{house} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
     \texttt{jannis} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
 \texttt{kddipums97} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
     \texttt{letter} &            Adam &              $1e-05$ &               $1e-03$ &      \texttt{False} &              &       & $18.4$ &                $4$ &              $64$ &               $.05$ &                 &                  $1.00$ &              $.40$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
     \texttt{online} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.20$ &                 &                  $1.67$ &              $.50$ &                                                            \\
    \texttt{phoneme} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
        \texttt{pol} &           AdamW &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &  $8.4$ &                $4$ &             $256$ &               $.05$ &               $.10$ &                  $1.67$ &              $.40$ &                                                            \\
         \texttt{rl} &            Adam &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &  $1.4$ &                $2$ &             $320$ &               $.30$ &                 &                  $1.67$ &              $.15$ &                                                            \\
  \texttt{upselling} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &  $2.0$ &                $1$ &              $64$ &               $.15$ &                 &                  $1.33$ &              $.45$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} &     $o$ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &             SGD &              $1e-02$ &               $1e-04$ &      \texttt{False} &            $.96$ &     \texttt{True} & $748.4$ &                $4$ &             $128$ &            $192$ &                $2.00$ &                  $.20$ &                 $.40$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &             SGD &              $1e-01$ &               $1e-03$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $1.2$ &                $4$ &              $64$ &            $192$ &                $1.00$ &                  $.45$ &                 $.30$ &                                                       \\
   \texttt{giveme} &           AdamW &              $1e-05$ &               $1e-04$ &       \texttt{True} &              &       &   $2.0$ &                $1$ &             $384$ &            $512$ &                $4.00$ &                  $.40$ &                 $.30$ &                                                       \\
   \texttt{helena} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &  $89.0$ &                $1$ &             $384$ &            $448$ &                $3.00$ &                  $.40$ &                 $.25$ &                                                       \\
   \texttt{indian} &             SGD &              $1e-01$ &               $1e-03$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $3.2$ &                $4$ &              $64$ &            $192$ &                $1.00$ &                  $.40$ &                 $.30$ &                                                       \\
\texttt{miniboone} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &   $2.0$ &                $1$ &             $384$ &            $448$ &                $3.00$ &                  $.40$ &                 $.25$ &                                                       \\
\texttt{ucicredit} &           AdamW &              $1e-05$ &               $1e-04$ &       \texttt{True} &              &       &   $2.0$ &                $1$ &             $448$ &            $448$ &                $3.00$ &                  $.30$ &                 $.25$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} &     $o$ & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &            Adam &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &   $2.8$ &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &   $4.0$ &             \texttt{False} &                                                          \\
   \texttt{breastmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $5.0$ &             \texttt{False} &                                                          \\
    \texttt{chestmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $5.0$ &             \texttt{False} &                                                          \\
    \texttt{dermamnist} &           AdamW &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &   $3.4$ &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $31.4$ &              \texttt{True} &                                                          \\
      \texttt{octmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $5.0$ &             \texttt{False} &                                                          \\
   \texttt{organamnist} &             SGD &              $1e-02$ &               $1e-03$ &      \texttt{False} &            $.93$ &     \texttt{True} &   $7.2$ &              \texttt{True} &                                                          \\
   \texttt{organcmnist} &             SGD &              $1e-02$ &               $1e-03$ &      \texttt{False} &            $.94$ &     \texttt{True} &   $6.8$ &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &           AdamW &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &   $5.8$ &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &             SGD &              $1e-01$ &               $1e-03$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $1.2$ &              \texttt{True} &                                                          \\
     \texttt{pathmnist} &            Adam &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &   $3.4$ &              \texttt{True} &                                                          \\
\texttt{pneumoniamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &   $5.0$ &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &           AdamW &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &   $2.8$ &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       & $161.0$ &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &             SGD &              $1e-03$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &   $8.0$ &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &           AdamW &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &   $2.0$ &             \texttt{False} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} &   $o$ & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &             SGD &              $1e-04$ &               $1e-05$ &      \texttt{False} &            $.99$ &     \texttt{True} & $7.8$ &    \texttt{True} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &             SGD &              $1e-02$ &               $1e-03$ &      \texttt{False} &            $.91$ &     \texttt{True} & $1.4$ &    \texttt{True} &                                                 \\
 \texttt{cifar10} &             SGD &              $1e-02$ &               $1e-03$ &      \texttt{False} &            $.91$ &     \texttt{True} & $5.2$ &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \SAT{}, divided by architectures.}
\label{tab:best_perf_sat}
\begin{tabular}{cccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &           AdamW &              $1e-05$ &               $1e-05$ &       \texttt{True} &              &       &  $45$ &   $.97$ &                $3$ &             $128$ &               $.40$ &                 &                  $1.67$ &               & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &  $45$ &   $.92$ &                $2$ &             $128$ &               $.50$ &                 &                  $2.33$ &              $.45$ &                                                            \\
    \texttt{covtype} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.95$ &                $4$ &             $320$ &               $.15$ &                 &                  $.67$ &              $.05$ &                                                            \\
\texttt{electricity} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &  $15$ &   $.98$ &                $3$ &             $128$ &               $.45$ &                 &                  $1.00$ &              $.10$ &                                                            \\
        \texttt{eye} &           AdamW &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $45$ &   $.97$ &                $3$ &             $256$ &               $.20$ &                 &                  $2.33$ &               &                                                            \\
      \texttt{heloc} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &  $45$ &   $.92$ &                $2$ &             $192$ &               $.45$ &                 &                  $2.00$ &              $.45$ &                                                            \\
      \texttt{higgs} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &  $60$ &   $.99$ &                $2$ &             $192$ &               $.15$ &               $.10$ &                  $1.00$ &               &                                                            \\
      \texttt{house} &           AdamW &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $15$ &   $.97$ &                $1$ &             $384$ &               $.25$ &               $.20$ &                  $1.00$ &              $.35$ &                                                            \\
     \texttt{jannis} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.94$ &                $3$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
 \texttt{kddipums97} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.93$ &                $4$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
     \texttt{letter} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.92$ &                $4$ &             $256$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.94$ &                $4$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
     \texttt{online} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &  $60$ &   $.99$ &                $2$ &             $192$ &               $.15$ &               $.10$ &                  $1.00$ &               &                                                            \\
    \texttt{phoneme} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.93$ &                $4$ &              $64$ &               $.30$ &                 &                  $1.00$ &              $.30$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.93$ &                $4$ &             $192$ &               $.15$ &                 &                  $1.00$ &              $.30$ &                                                            \\
         \texttt{rl} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.98$ &                $3$ &              $64$ &               $.45$ &                 &                  $1.00$ &              $.10$ &                                                            \\
  \texttt{upselling} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.93$ &                $4$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &   $0$ &   $.93$ &                $2$ &             $320$ &            $384$ &                $3.00$ &                  $.50$ &                 $.50$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-02$ &               $1e-04$ &       \texttt{True} &              &       &  $15$ &   $.93$ &                $2$ &             $320$ &            $320$ &                $2.00$ &                  $.45$ &                 $.15$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &  $30$ &   $.91$ &                $1$ &             $512$ &            $192$ &                $3.00$ &                  $.15$ &                 $.25$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &  $30$ &    $.9$ &                $4$ &             $192$ &            $128$ &                $2.00$ &                  $.45$ &                 $.15$ &                                                       \\
   \texttt{indian} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &   $0$ &   $.98$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &   $0$ &   $.98$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
\texttt{ucicredit} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &   $0$ &   $.98$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &             SGD &              $1e-02$ &               $1e-05$ &      \texttt{False} &            $.92$ &    \texttt{False} &   $0$ &   $.99$ &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $60$ &    $.9$ &              \texttt{True} &                                                          \\
   \texttt{breastmnist} &           AdamW &              $1e-05$ &               $1e-03$ &      \texttt{False} &              &       &   $0$ &   $.91$ &             \texttt{False} &                                                          \\
    \texttt{chestmnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $60$ &    $.9$ &              \texttt{True} &                                                          \\
    \texttt{dermamnist} &           AdamW &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &  $30$ &   $.94$ &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $45$ &    $.9$ &             \texttt{False} &                                                          \\
      \texttt{octmnist} &           AdamW &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &  $60$ &   $.92$ &              \texttt{True} &                                                          \\
   \texttt{organamnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.98$ &              \texttt{True} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.91$ &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &  $45$ &   $.93$ &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &           AdamW &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $45$ &   $.91$ &             \texttt{False} &                                                          \\
     \texttt{pathmnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.91$ &              \texttt{True} &                                                          \\
\texttt{pneumoniamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &  $60$ &    $.9$ &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &           AdamW &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.95$ &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &  $15$ &   $.93$ &              \texttt{True} &                                                          \\
   \texttt{tissuemnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.91$ &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &             SGD &              $1e-02$ &               $1e-03$ &      \texttt{False} &             $.9$ &     \texttt{True} &  $30$ &   $.92$ &             \texttt{False} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &    $.9$ &    \texttt{True} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $45$ &    $.9$ &    \texttt{True} &                                                 \\
 \texttt{cifar10} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $45$ &   $.93$ &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \SATEM{}, divided by architectures.}
\label{tab:best_perf_sat_te}
\begin{tabular}{ccccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & $ \beta $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &             SGD &              $1e-04$ &               $1e-06$ &      \texttt{False} &            $.95$ &     \texttt{True} &  $45$ &    $.9$ &    $.01$ &                $3$ &             $256$ &               $.50$ &                &                  $2.67$ &              $.50$ & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.96$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
    \texttt{covtype} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &  $30$ &   $.98$ &   $.001$ &                $3$ &             $320$ &                &                 &                  $2.33$ &              $.10$ &                                                            \\
\texttt{electricity} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &  $30$ &   $.96$ &   $.001$ &                $3$ &             $320$ &               $.05$ &                 &                  $2.33$ &              $.10$ &                                                            \\
        \texttt{eye} &           AdamW &              $1e-05$ &               $1e-04$ &       \texttt{True} &              &       &  $30$ &   $.91$ &    $.01$ &                $2$ &             $448$ &               $.30$ &                 &                  $1.33$ &              $.15$ &                                                            \\
      \texttt{heloc} &           AdamW &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &  $30$ &   $.92$ &  $.0001$ &                $2$ &             $384$ &               $.10$ &               $.15$ &                  $2.33$ &              $.50$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &  $30$ &   $.98$ &   $.001$ &                $2$ &             $448$ &               $.10$ &                 &                  $1.67$ &              $.30$ &                                                            \\
      \texttt{house} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.96$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
     \texttt{jannis} &           AdamW &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &  $30$ &   $.97$ &  $.0001$ &                $3$ &             $448$ &               $.10$ &                 &                  $2.00$ &              $.25$ &                                                            \\
 \texttt{kddipums97} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.95$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
     \texttt{letter} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &  $30$ &   $.96$ &   $.001$ &                $3$ &             $384$ &                &                 &                  $2.67$ &               &                                                            \\
      \texttt{magic} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.94$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
     \texttt{online} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.96$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
    \texttt{phoneme} &           AdamW &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.99$ &    $.01$ &                $3$ &             $320$ &               $.20$ &                 &                  $2.67$ &              $.40$ &                                                            \\
        \texttt{pol} &           AdamW &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $30$ &   $.98$ &  $.0001$ &                $3$ &             $448$ &               $.15$ &                 &                  $2.00$ &              $.30$ &                                                            \\
         \texttt{rl} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.97$ &  $.0001$ &                $1$ &             $512$ &               $.50$ &                 &                  $1.33$ &              $.15$ &                                                            \\
  \texttt{upselling} &           AdamW &              $1e-05$ &               $1e-06$ &       \texttt{True} &              &       &  $30$ &   $.99$ &  $.0001$ &                $3$ &             $448$ &               $.10$ &                 &                  $2.00$ &              $.30$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & $ \beta $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &             SGD &              $1e-01$ &               $1e-04$ &      \texttt{False} &            $.93$ &    \texttt{False} &  $15$ &   $.91$ &   $.001$ &                $3$ &             $192$ &            $512$ &                $4.00$ &                  $.10$ &                 $.25$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.94$ &   $.001$ &                $1$ &             $384$ &            $256$ &                $1.00$ &                  $.30$ &                 $.05$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &                $2$ &             $384$ &            $256$ &                $2.00$ &                  $.25$ &                 $.05$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.95$ &  $.0001$ &                $2$ &             $384$ &            $256$ &                $2.00$ &                  $.25$ &                 $.05$ &                                                       \\
   \texttt{indian} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.94$ &   $.001$ &                $2$ &             $384$ &            $256$ &                $1.00$ &                  $.30$ &                 $.05$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &  $15$ &   $.94$ &   $.001$ &                $1$ &             $384$ &            $256$ &                $1.00$ &                  $.30$ &                 $.05$ &                                                       \\
\texttt{ucicredit} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.92$ &   $.001$ &                $2$ &             $512$ &            $128$ &                $3.00$ &                  $.40$ &                 $.10$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & $ \beta $ & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &             SGD &              $1e-01$ &               $1e-05$ &      \texttt{False} &            $.96$ &     \texttt{True} &  $60$ &   $.98$ &  $.0001$ &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.96$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{breastmnist} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &  $45$ &    $.9$ &    $.01$ &             \texttt{False} &                                                          \\
    \texttt{chestmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{dermamnist} &             SGD &              $1e-04$ &               $1e-05$ &      \texttt{False} &            $.99$ &     \texttt{True} &  $60$ &   $.98$ &  $.0001$ &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &    $.9$ &    $.01$ &              \texttt{True} &                                                          \\
      \texttt{octmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organamnist} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.96$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &  $60$ &   $.96$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organsmnist} &             SGD &              $1e-02$ &               $1e-05$ &      \texttt{False} &            $.95$ &     \texttt{True} &  $60$ &   $.98$ &  $.0001$ &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &            $.93$ &     \texttt{True} &   $0$ &   $.98$ &  $.0001$ &             \texttt{False} &                                                          \\
     \texttt{pathmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.95$ &  $.0001$ &             \texttt{False} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.94$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &             \texttt{False} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &  $15$ &   $.98$ &   $.001$ &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &   $0$ &   $.96$ &  $.0001$ &             \texttt{False} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $E_s$ & $\gamma$ & $ \beta $ & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &   $0$ &   $.93$ &  $.0001$ &   \texttt{False} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &             SGD &              $1e-01$ &               $1e-05$ &      \texttt{False} &            $.96$ &     \texttt{True} &  $60$ &   $.98$ &  $.0001$ &    \texttt{True} &                                                 \\
 \texttt{cifar10} &             SGD &              $1e-01$ &               $1e-04$ &      \texttt{False} &            $.93$ &     \texttt{True} &  $60$ &   $.98$ &  $.0001$ &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \SelNet{}, divided by architectures.}
\label{tab:best_perf_selnet}
\begin{tabular}{cccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &           AdamW &              $1e-05$ &               $1e-06$ &       \texttt{True} &              &       &      $32$ &     $.65$ &                $3$ &             $192$ &               $.40$ &                 &                  $2.00$ &               & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &      $64$ &     $.75$ &                $2$ &             $192$ &               $.15$ &               $.10$ &                  $1.00$ &               &                                                            \\
    \texttt{covtype} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.25$ &                $3$ &             $384$ &               $.10$ &                 &                  $.67$ &               &                                                            \\
\texttt{electricity} &            Adam &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &      $64$ &     $.75$ &                $2$ &             $192$ &               $.05$ &               $.05$ &                  $1.00$ &               &                                                            \\
        \texttt{eye} &           AdamW &              $1e-05$ &               $1e-06$ &       \texttt{True} &              &       &      $32$ &     $.70$ &                $3$ &             $320$ &               $.35$ &                 &                  $2.67$ &              $.05$ &                                                            \\
      \texttt{heloc} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.70$ &                $2$ &              $64$ &               $.50$ &                 &                  $1.33$ &              $.10$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &      $64$ &     $.65$ &                $3$ &             $192$ &               $.25$ &                 &                  $2.67$ &               &                                                            \\
      \texttt{house} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &      $64$ &     $.75$ &                $2$ &             $192$ &               $.15$ &               $.10$ &                  $1.00$ &               &                                                            \\
     \texttt{jannis} &           AdamW &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &      $64$ &     $.35$ &                $2$ &             $256$ &               $.50$ &                 &                  $2.33$ &              $.50$ &                                                            \\
 \texttt{kddipums97} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.70$ &                $3$ &              $64$ &               $.50$ &                 &                  $1.33$ &              $.10$ &                                                            \\
     \texttt{letter} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.40$ &                $4$ &             $320$ &               $.10$ &                 &                  $.67$ &              $.20$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &      $32$ &     $.55$ &                $3$ &             $256$ &               $.15$ &                &                  $.67$ &              $.10$ &                                                            \\
     \texttt{online} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &      $64$ &     $.70$ &                $2$ &             $192$ &               $.15$ &               $.20$ &                  $1.00$ &               &                                                            \\
    \texttt{phoneme} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.35$ &                $3$ &             $320$ &               $.10$ &                 &                  $1.33$ &              $.30$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &      $64$ &     $.75$ &                $2$ &             $192$ &               $.15$ &               $.10$ &                  $1.00$ &               &                                                            \\
         \texttt{rl} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.70$ &                $3$ &              $64$ &               $.50$ &                 &                  $1.00$ &              $.10$ &                                                            \\
  \texttt{upselling} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.45$ &                $4$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &      $32$ &     $.25$ &                $4$ &             $128$ &            $128$ &                $2.00$ &                  $.50$ &                 $.05$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &       $8$ &     $.70$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &       $8$ &     $.70$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &      $32$ &     $.25$ &                $4$ &             $128$ &            $128$ &                $2.00$ &                  $.50$ &                 $.10$ &                                                       \\
   \texttt{indian} &           AdamW &              $1e-02$ &               $1e-04$ &       \texttt{True} &              &       &      $32$ &     $.65$ &                $2$ &             $256$ &            $320$ &                $2.00$ &                  $.40$ &                 $.15$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &       $8$ &     $.70$ &                $4$ &             $512$ &            $192$ &                $1.00$ &                  $.10$ &                 $.20$ &                                                       \\
\texttt{ucicredit} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &      $32$ &     $.25$ &                $4$ &             $192$ &             $64$ &                $2.00$ &                  $.45$ &                 $.10$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.94$ &     \texttt{True} &      $32$ &     $.55$ &             \texttt{False} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.99$ &     \texttt{True} &      $32$ &     $.45$ &             \texttt{False} &                                                          \\
   \texttt{breastmnist} &           AdamW &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &      $32$ &     $.45$ &              \texttt{True} &                                                          \\
    \texttt{chestmnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $64$ &     $.25$ &              \texttt{True} &                                                          \\
    \texttt{dermamnist} &           AdamW &              $1e-05$ &               $1e-03$ &      \texttt{False} &              &       &      $16$ &     $.30$ &             \texttt{False} &                                                          \\
       \texttt{food101} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &      $32$ &     $.50$ &             \texttt{False} &                                                          \\
      \texttt{octmnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.30$ &              \texttt{True} &                                                          \\
   \texttt{organamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.94$ &     \texttt{True} &      $32$ &     $.50$ &             \texttt{False} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $32$ &     $.30$ &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.25$ &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &           AdamW &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.25$ &             \texttt{False} &                                                          \\
     \texttt{pathmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.93$ &     \texttt{True} &      $64$ &     $.60$ &             \texttt{False} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.30$ &              \texttt{True} &                                                          \\
   \texttt{retinamnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.30$ &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $64$ &     $.25$ &              \texttt{True} &                                                          \\
   \texttt{tissuemnist} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.30$ &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.45$ &              \texttt{True} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $64$ &     $.25$ &    \texttt{True} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &            Adam &              $1e-02$ &               $1e-06$ &       \texttt{True} &              &       &      $32$ &     $.25$ &    \texttt{True} &                                                 \\
 \texttt{cifar10} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.70$ &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \SelNetEM{}, divided by architectures.}
\label{tab:best_perf_selnet_te}
\begin{tabular}{ccccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & $ \beta $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &           AdamW &              $1e-02$ &               $1e-05$ &       \texttt{True} &              &       &      $16$ &     $.25$ &  $.0001$ &                $2$ &             $384$ &               $.15$ &                &                  $2.33$ &              $.50$ & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &           AdamW &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.75$ &  $.0001$ &                $3$ &             $448$ &               $.15$ &                 &                  $2.00$ &              $.30$ &                                                            \\
    \texttt{covtype} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &      $16$ &     $.60$ &   $.001$ &                $3$ &             $320$ &               $.05$ &                 &                  $2.33$ &              $.10$ &                                                            \\
\texttt{electricity} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.45$ &  $.0001$ &                $4$ &             $256$ &               $.10$ &                 &                  $1.00$ &              $.35$ &                                                            \\
        \texttt{eye} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &      $64$ &     $.25$ &    $.01$ &                $1$ &             $448$ &               $.25$ &                 &                  $1.67$ &              $.20$ &                                                            \\
      \texttt{heloc} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &      $64$ &     $.25$ &    $.01$ &                $1$ &             $448$ &               $.35$ &                 &                  $1.33$ &              $.15$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &      $64$ &     $.35$ &    $.01$ &                $1$ &             $384$ &               $.20$ &                 &                  $1.33$ &              $.10$ &                                                            \\
      \texttt{house} &           AdamW &              $1e-05$ &               $1e-05$ &       \texttt{True} &              &       &       $8$ &     $.50$ &  $.0001$ &                $3$ &             $384$ &               $.20$ &                 &                  $1.33$ &               &                                                            \\
     \texttt{jannis} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.60$ &  $.0001$ &                $1$ &             $512$ &               $.50$ &                 &                  $1.67$ &              $.15$ &                                                            \\
 \texttt{kddipums97} &           AdamW &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.70$ &  $.0001$ &                $3$ &             $448$ &               $.10$ &                 &                  $2.00$ &              $.30$ &                                                            \\
     \texttt{letter} &           AdamW &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.70$ &  $.0001$ &                $3$ &             $448$ &               $.10$ &                 &                  $2.00$ &              $.35$ &                                                            \\
      \texttt{magic} &           AdamW &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.75$ &  $.0001$ &                $3$ &             $448$ &               $.15$ &                 &                  $2.00$ &              $.25$ &                                                            \\
     \texttt{online} &           AdamW &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.75$ &  $.0001$ &                $3$ &             $448$ &               $.15$ &                 &                  $2.00$ &              $.30$ &                                                            \\
    \texttt{phoneme} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.50$ &  $.0001$ &                $4$ &             $192$ &               $.15$ &                 &                  $1.00$ &              $.35$ &                                                            \\
        \texttt{pol} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &      $16$ &     $.65$ &   $.001$ &                $3$ &             $320$ &                &                 &                  $2.67$ &               &                                                            \\
         \texttt{rl} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.55$ &  $.0001$ &                $1$ &             $512$ &               $.45$ &                 &                  $1.33$ &              $.10$ &                                                            \\
  \texttt{upselling} &           AdamW &              $1e-05$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.70$ &  $.0001$ &                $3$ &             $448$ &               $.10$ &                 &                  $2.00$ &              $.30$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & $ \beta $ & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &             SGD &              $1e-01$ &               $1e-05$ &      \texttt{False} &            $.99$ &    \texttt{False} &      $64$ &     $.65$ &  $.0001$ &                $4$ &             $320$ &            $384$ &                $3.00$ &                  $.15$ &                 $.05$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.55$ &  $.0001$ &                $1$ &             $320$ &            $320$ &                $1.00$ &                  $.30$ &                 $.05$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.45$ &  $.0001$ &                $1$ &             $384$ &            $256$ &                $1.00$ &                  $.25$ &                 $.05$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.50$ &  $.0001$ &                $2$ &             $448$ &            $192$ &                $1.00$ &                  $.25$ &                 $.05$ &                                                       \\
   \texttt{indian} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.35$ &   $.001$ &                $2$ &             $512$ &            $128$ &                $3.00$ &                  $.40$ &                 $.05$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.45$ &  $.0001$ &                $2$ &             $384$ &            $256$ &                $2.00$ &                  $.25$ &                 $.05$ &                                                       \\
\texttt{ucicredit} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &      $16$ &     $.45$ &   $.001$ &                $1$ &             $384$ &            $256$ &                $1.00$ &                  $.30$ &                 $.05$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & $ \beta $ & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &             SGD &              $1e-03$ &               $1e-05$ &      \texttt{False} &            $.93$ &    \texttt{False} &      $64$ &     $.35$ &  $.0001$ &             \texttt{False} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.55$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{breastmnist} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.40$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{chestmnist} &             SGD &              $1e-02$ &               $1e-05$ &      \texttt{False} &            $.93$ &     \texttt{True} &      $64$ &     $.30$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{dermamnist} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.60$ &  $.0001$ &             \texttt{False} &                                                          \\
       \texttt{food101} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.40$ &  $.0001$ &             \texttt{False} &                                                          \\
      \texttt{octmnist} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.60$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organamnist} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.55$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.55$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.60$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{oxfordpets} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &            $.95$ &    \texttt{False} &      $32$ &     $.50$ &  $.0001$ &             \texttt{False} &                                                          \\
     \texttt{pathmnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.55$ &  $.0001$ &             \texttt{False} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $64$ &     $.55$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &            Adam &              $1e-02$ &               $1e-06$ &      \texttt{False} &              &       &       $8$ &     $.60$ &  $.0001$ &             \texttt{False} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.40$ &  $.0001$ &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.40$ &  $.0001$ &             \texttt{False} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.60$ &  $.0001$ &             \texttt{False} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & $\lambda$ & $ \alpha $ & $ \beta $ & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &       $8$ &     $.40$ &  $.0001$ &   \texttt{False} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &      $16$ &     $.65$ &  $.0001$ &   \texttt{False} &                                                 \\
 \texttt{cifar10} &             SGD &              $1e-02$ &               $1e-03$ &       \texttt{True} &            $.99$ &     \texttt{True} &      $32$ &     $.50$ &   $.001$ &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \SR{}, divided by architectures.}
\label{tab:best_perf_plugin}
\begin{tabular}{cccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &             SGD &              $1e-03$ &               $1e-04$ &      \texttt{False} &            $.91$ &    \texttt{False} &                $4$ &             $128$ &               $.25$ &                 &                  $1.00$ &              $.30$ & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &                $1$ &             $320$ &               $.10$ &               $.10$ &                  $2.00$ &              $.25$ &                                                            \\
    \texttt{covtype} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                $3$ &             $384$ &               $.45$ &                 &                  $2.33$ &              $.35$ &                                                            \\
\texttt{electricity} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                $3$ &             $384$ &               $.45$ &                 &                  $2.33$ &              $.35$ &                                                            \\
        \texttt{eye} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $1$ &             $384$ &               $.15$ &               $.05$ &                  $2.33$ &              $.20$ &                                                            \\
      \texttt{heloc} &             SGD &              $1e-04$ &               $1e-04$ &      \texttt{False} &            $.93$ &     \texttt{True} &                $4$ &             $128$ &               $.30$ &                 &                  $1.00$ &              $.30$ &                                                            \\
      \texttt{higgs} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $2$ &             $384$ &               $.20$ &                &                  $2.00$ &              $.15$ &                                                            \\
      \texttt{house} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $2$ &             $320$ &               $.20$ &               $.10$ &                  $2.00$ &              $.15$ &                                                            \\
     \texttt{jannis} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $2$ &             $384$ &               $.25$ &               $.15$ &                  $2.00$ &              $.20$ &                                                            \\
 \texttt{kddipums97} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $4$ &             $320$ &               $.35$ &               $.20$ &                  $1.00$ &              $.10$ &                                                            \\
     \texttt{letter} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                $3$ &             $384$ &               $.45$ &                 &                  $2.33$ &              $.35$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &                $1$ &             $384$ &               $.10$ &                &                  $2.33$ &              $.30$ &                                                            \\
     \texttt{online} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                $1$ &             $384$ &               $.45$ &                 &                  $2.33$ &              $.35$ &                                                            \\
    \texttt{phoneme} &            Adam &              $1e-02$ &               $1e-04$ &      \texttt{False} &              &       &                $1$ &             $128$ &                &               $.05$ &                  $1.33$ &              $.45$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                $1$ &             $192$ &               $.05$ &               $.10$ &                  $1.67$ &              $.40$ &                                                            \\
         \texttt{rl} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                $3$ &             $512$ &               $.50$ &                 &                  $1.67$ &              $.30$ &                                                            \\
  \texttt{upselling} &             SGD &              $1e-02$ &               $1e-04$ &      \texttt{False} &            $.99$ &     \texttt{True} &                $4$ &              $64$ &               $.25$ &                 &                  $1.00$ &              $.20$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $4$ &             $192$ &            $320$ &                $4.00$ &                  $.10$ &                 $.20$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &                $4$ &             $256$ &             $64$ &                $3.00$ &                  $.40$ &                 $.30$ &                                                       \\
   \texttt{giveme} &           AdamW &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &                $3$ &              $64$ &            $256$ &                $2.00$ &                  $.30$ &                 $.40$ &                                                       \\
   \texttt{helena} &           AdamW &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                $3$ &             $192$ &            $320$ &                $4.00$ &                  $.10$ &                 $.20$ &                                                       \\
   \texttt{indian} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &                $4$ &             $256$ &             $64$ &                $3.00$ &                  $.40$ &                 $.30$ &                                                       \\
\texttt{miniboone} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &                $4$ &             $256$ &             $64$ &                $3.00$ &                  $.40$ &                 $.30$ &                                                       \\
\texttt{ucicredit} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                $3$ &             $192$ &            $128$ &                $2.00$ &                  $.25$ &                 $.35$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &             \texttt{False} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
   \texttt{breastmnist} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
    \texttt{chestmnist} &           AdamW &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
    \texttt{dermamnist} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &             \texttt{False} &                                                          \\
      \texttt{octmnist} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
   \texttt{organamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.93$ &     \texttt{True} &             \texttt{False} &                                                          \\
   \texttt{organcmnist} &           AdamW &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &             \texttt{False} &                                                          \\
    \texttt{oxfordpets} &            Adam &              $1e-02$ &               $1e-05$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
     \texttt{pathmnist} &             SGD &              $1e-02$ &               $1e-03$ &       \texttt{True} &            $.97$ &     \texttt{True} &             \texttt{False} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &              \texttt{True} &                                                          \\
   \texttt{retinamnist} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &             \texttt{False} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &             SGD &              $1e-03$ &               $1e-06$ &      \texttt{False} &            $.91$ &     \texttt{True} &   \texttt{False} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &   \texttt{False} &                                                 \\
 \texttt{cifar10} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \Sele{}, divided by architectures.}
\label{tab:best_perf_sele}
\begin{tabular}{cccccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &             SGD &              $1e-03$ &               $1e-06$ &       \texttt{True} &            $.93$ &     \texttt{True} &                AdamW &                   $1e-07$ &                   &            &                $4$ &             $256$ &               $.05$ &               $.10$ &                  $1.67$ &              $.40$ & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
    \texttt{covtype} &             SGD &              $1e-01$ &               $1e-06$ &       \texttt{True} &             $.9$ &    \texttt{False} &                AdamW &                   $1e-07$ &                   &            &                $4$ &             $256$ &               $.05$ &                &                  $1.33$ &              $.35$ &                                                            \\
\texttt{electricity} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $4$ &             $448$ &               $.10$ &               $.15$ &                  $1.67$ &              $.25$ &                                                            \\
        \texttt{eye} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
      \texttt{heloc} &            Adam &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &                  SGD &                   $1e-04$ &                 $.94$ &          \texttt{True} &                $1$ &             $128$ &               $.50$ &               $.05$ &                  $1.33$ &              $.15$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &                $3$ &             $192$ &               $.15$ &               $.10$ &                  $2.00$ &              $.40$ &                                                            \\
      \texttt{house} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
     \texttt{jannis} &             SGD &              $1e-03$ &               $1e-03$ &      \texttt{False} &            $.94$ &     \texttt{True} &                AdamW &                   $1e-07$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.20$ &                                                            \\
 \texttt{kddipums97} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
     \texttt{letter} &             SGD &              $1e-02$ &               $1e-05$ &      \texttt{False} &            $.95$ &     \texttt{True} &                  SGD &                   $1e-04$ &                 $.99$ &          \texttt{True} &                $2$ &             $320$ &               $.25$ &               $.05$ &                  $2.33$ &              $.40$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &                $3$ &             $128$ &               $.15$ &               $.20$ &                  $.67$ &              $.10$ &                                                            \\
     \texttt{online} &           AdamW &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                 Adam &                   $1e-04$ &                   &            &                $1$ &             $512$ &               $.50$ &                 &                  $2.67$ &              $.25$ &                                                            \\
    \texttt{phoneme} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                 Adam &                   $1e-04$ &                   &            &                $4$ &             $448$ &               $.10$ &               $.05$ &                  $1.67$ &              $.25$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &                  SGD &                   $1e-04$ &                 $.93$ &          \texttt{True} &                $2$ &             $384$ &               $.05$ &               $.05$ &                  $1.67$ &              $.30$ &                                                            \\
         \texttt{rl} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                 Adam &                   $1e-04$ &                   &            &                $4$ &             $448$ &               $.10$ &               $.05$ &                  $1.67$ &              $.25$ &                                                            \\
  \texttt{upselling} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &                $3$ &             $128$ &               $.35$ &                 &                  $2.67$ &              $.05$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &           AdamW &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                 $.92$ &          \texttt{True} &                $1$ &              $64$ &            $512$ &                $3.00$ &                  $.40$ &                 $.15$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-02$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-03$ &                   &            &                $2$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
   \texttt{giveme} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-03$ &                   &            &                $3$ &             $256$ &            $512$ &                $1.00$ &                  $.20$ &                 $.05$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &            $512$ &                $4.00$ &                  $.50$ &                 $.25$ &                                                       \\
   \texttt{indian} &            Adam &              $1e-02$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-03$ &                   &            &                $2$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
\texttt{miniboone} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-06$ &                   &            &                $3$ &             $320$ &            $512$ &                $1.00$ &                  $.20$ &                 $.15$ &                                                       \\
\texttt{ucicredit} &            Adam &              $1e-02$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-03$ &                   &            &                $2$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &             SGD &              $1e-01$ &               $1e-03$ &       \texttt{True} &            $.95$ &    \texttt{False} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-02$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-04$ &                 $.94$ &          \texttt{True} &              \texttt{True} &                                                          \\
   \texttt{breastmnist} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{chestmnist} &             SGD &              $1e-01$ &               $1e-05$ &       \texttt{True} &            $.95$ &    \texttt{False} &                 Adam &                   $1e-03$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{dermamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.93$ &    \texttt{False} &                 Adam &                   $1e-04$ &                   &            &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-04$ &                   &            &             \texttt{False} &                                                          \\
      \texttt{octmnist} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &            $.96$ &     \texttt{True} &                 Adam &                   $1e-04$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.94$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
     \texttt{pathmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.93$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
\texttt{pneumoniamnist} &           AdamW &              $1e-03$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-06$ &                   &            &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.99$ &    \texttt{False} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-03$ &                   &            &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &            $.94$ &     \texttt{True} &                 Adam &                   $1e-03$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-04$ &                 $.93$ &          \texttt{True} &              \texttt{True} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &           AdamW &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &   \texttt{False} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &           AdamW &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                 $.95$ &          \texttt{True} &    \texttt{True} &                                                 \\
 \texttt{cifar10} &           AdamW &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                 $.99$ &          \texttt{True} &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \Reg{}, divided by architectures.}
\label{tab:best_perf_reg}
\begin{tabular}{cccccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &           AdamW &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-05$ &                 $.92$ &          \texttt{True} &                $2$ &             $128$ &               $.50$ &                 &                  $2.33$ &              $.45$ & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &             SGD &              $1e-01$ &               $1e-06$ &       \texttt{True} &             $.9$ &    \texttt{False} &                AdamW &                   $1e-07$ &                   &            &                $4$ &             $256$ &               $.10$ &                &                  $1.67$ &              $.35$ &                                                            \\
    \texttt{covtype} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-06$ &                   &            &                $2$ &             $320$ &               $.10$ &               $.05$ &                  $.67$ &              $.15$ &                                                            \\
\texttt{electricity} &             SGD &              $1e-03$ &               $1e-04$ &       \texttt{True} &            $.99$ &     \texttt{True} &                AdamW &                   $1e-04$ &                   &            &                $2$ &             $128$ &               $.35$ &                 &                  $1.33$ &               &                                                            \\
        \texttt{eye} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
      \texttt{heloc} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &                  SGD &                   $1e-04$ &                  $.9$ &         \texttt{False} &                $1$ &              $64$ &               $.15$ &                 &                  $2.00$ &              $.25$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-04$ &                  $.9$ &          \texttt{True} &                $2$ &              $64$ &               $.50$ &                 &                  $2.33$ &              $.50$ &                                                            \\
      \texttt{house} &             SGD &              $1e-03$ &               $1e-04$ &      \texttt{False} &            $.95$ &     \texttt{True} &                AdamW &                   $1e-06$ &                   &            &                $3$ &             $256$ &               $.35$ &               $.05$ &                  $.67$ &              $.15$ &                                                            \\
     \texttt{jannis} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &                $4$ &              $64$ &               $.25$ &                 &                  $2.67$ &              $.05$ &                                                            \\
 \texttt{kddipums97} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-07$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
     \texttt{letter} &             SGD &              $1e-02$ &               $1e-04$ &      \texttt{False} &             $.9$ &    \texttt{False} &                AdamW &                   $1e-06$ &                   &            &                $3$ &             $320$ &               $.20$ &               $.05$ &                  $1.67$ &              $.25$ &                                                            \\
      \texttt{magic} &            Adam &              $1e-04$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &                $3$ &             $128$ &               $.05$ &                &                  $1.33$ &              $.25$ &                                                            \\
     \texttt{online} &            Adam &              $1e-04$ &               $1e-06$ &      \texttt{False} &              &       &                 Adam &                   $1e-04$ &                   &            &                $1$ &             $384$ &               $.30$ &                &                  $2.67$ &              $.20$ &                                                            \\
    \texttt{phoneme} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-05$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &                AdamW &                   $1e-06$ &                   &            &                $4$ &             $320$ &               $.25$ &                 &                  $2.00$ &              $.05$ &                                                            \\
         \texttt{rl} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &                $2$ &             $128$ &               $.10$ &                 &                  $.67$ &              $.30$ &                                                            \\
  \texttt{upselling} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &            Adam &              $1e-03$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-06$ &                   &            &                $3$ &             $128$ &            $512$ &                $4.00$ &                  $.50$ &                 $.45$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &             SGD &              $1e-01$ &               $1e-06$ &       \texttt{True} &            $.99$ &    \texttt{False} &                AdamW &                   $1e-07$ &                   &            &                $4$ &             $256$ &             $64$ &                $3.00$ &                  $.45$ &                 $.30$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                AdamW &                   $1e-04$ &                   &            &                $4$ &             $512$ &            $192$ &                $2.00$ &                  $.15$ &                 $.15$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &                  SGD &                   $1e-06$ &                 $.99$ &         \texttt{False} &                $3$ &             $192$ &            $320$ &                $3.00$ &                  $.25$ &                 $.05$ &                                                       \\
   \texttt{indian} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-03$ &                   &            &                $3$ &             $256$ &            $512$ &                $1.00$ &                  $.10$ &                 $.05$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-04$ &               $1e-03$ &       \texttt{True} &              &       &                  SGD &                   $1e-05$ &                 $.97$ &         \texttt{False} &                $3$ &             $256$ &            $384$ &                $3.00$ &                  $.25$ &                  &                                                       \\
\texttt{ucicredit} &           AdamW &              $1e-05$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-07$ &                   &            &                $3$ &             $192$ &            $512$ &                $1.00$ &                  $.15$ &                  &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &            Adam &              $1e-02$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-06$ &                  $.9$ &         \texttt{False} &              \texttt{True} &                                                          \\
   \texttt{breastmnist} &            Adam &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                AdamW &                   $1e-03$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{chestmnist} &           AdamW &              $1e-02$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-07$ &                   &            &             \texttt{False} &                                                          \\
    \texttt{dermamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.99$ &    \texttt{False} &                 Adam &                   $1e-04$ &                   &            &              \texttt{True} &                                                          \\
       \texttt{food101} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
      \texttt{octmnist} &             SGD &              $1e-02$ &               $1e-05$ &       \texttt{True} &            $.99$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organamnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-05$ &                 $.98$ &          \texttt{True} &              \texttt{True} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{oxfordpets} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-04$ &                   &            &              \texttt{True} &                                                          \\
     \texttt{pathmnist} &             SGD &              $1e-01$ &               $1e-05$ &       \texttt{True} &            $.97$ &     \texttt{True} &                 Adam &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                  $.9$ &         \texttt{False} &              \texttt{True} &                                                          \\
   \texttt{retinamnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.99$ &    \texttt{False} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-03$ &                   &            &             \texttt{False} &                                                          \\
   \texttt{tissuemnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &            $.97$ &    \texttt{False} &                 Adam &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-03$ &               $1e-06$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                 $.97$ &          \texttt{True} &              \texttt{True} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &    \texttt{True} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &            Adam &              $1e-02$ &               $1e-05$ &      \texttt{False} &              &       &                AdamW &                   $1e-04$ &                   &            &    \texttt{True} &                                                 \\
 \texttt{cifar10} &           AdamW &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &                  SGD &                   $1e-03$ &                 $.99$ &         \texttt{False} &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}}

44
\begin{sidewaystable}[h!]
\centering
\setlength\tabcolsep{1.5pt}
\fontsize{9}{9}\selectfont
\resizebox{!}{\textheight}{
\
\caption{Best configurations for \CN{}, divided by architectures.}
\label{tab:best_perf_cn}
\begin{tabular}{cccccccccccccccccc}
\toprule
             Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{att.\_drop.} & \texttt{res.\_drop.} & \texttt{d\_ffn\_factor} & \texttt{ffn\_drop.} &                                                      Arch. \\
\midrule
      \texttt{adult} &            Adam &              $1e-05$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-06$ &                   &            &                $4$ &              $64$ &               $.50$ &                 &                  $2.33$ &               & \multirow{17}{*}{\rotatebox[origin=c]{-90}{FTTransformer}} \\
    \texttt{compass} &            Adam &              $1e-03$ &               $1e-05$ &       \texttt{True} &              &       &                AdamW &                   $1e-06$ &                   &            &                $2$ &              $64$ &               $.40$ &                 &                  $2.00$ &              $.15$ &                                                            \\
    \texttt{covtype} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                 Adam &                   $1e-05$ &                   &            &                $2$ &             $448$ &               $.10$ &               $.15$ &                  $2.00$ &              $.35$ &                                                            \\
\texttt{electricity} &            Adam &              $1e-05$ &               $1e-06$ &      \texttt{False} &              &       &                 Adam &                   $1e-05$ &                   &            &                $4$ &             $448$ &               $.10$ &               $.05$ &                  $1.67$ &              $.25$ &                                                            \\
        \texttt{eye} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-06$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
      \texttt{heloc} &           AdamW &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-06$ &                 $.92$ &          \texttt{True} &                $2$ &             $128$ &               $.50$ &                 &                  $2.33$ &              $.45$ &                                                            \\
      \texttt{higgs} &           AdamW &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
      \texttt{house} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
     \texttt{jannis} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
 \texttt{kddipums97} &           AdamW &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.25$ &                                                            \\
     \texttt{letter} &             SGD &              $1e-03$ &               $1e-03$ &      \texttt{False} &            $.97$ &     \texttt{True} &                AdamW &                   $1e-05$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
      \texttt{magic} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
     \texttt{online} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
    \texttt{phoneme} &           AdamW &              $1e-03$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $512$ &               $.40$ &                 &                  $2.67$ &              $.30$ &                                                            \\
        \texttt{pol} &            Adam &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &                 Adam &                   $1e-05$ &                   &            &                $4$ &             $384$ &               $.05$ &               $.20$ &                  $2.00$ &              $.25$ &                                                            \\
         \texttt{rl} &           AdamW &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                 Adam &                   $1e-06$ &                   &            &                $1$ &             $448$ &               $.40$ &                 &                  $2.67$ &              $.25$ &                                                            \\
  \texttt{upselling} &             SGD &              $1e-04$ &               $1e-03$ &      \texttt{False} &            $.96$ &     \texttt{True} &                AdamW &                   $1e-06$ &                   &            &                $3$ &             $128$ &               $.35$ &                &                  $.67$ &              $.15$ &                                                            \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{cccccccccccccccccc}
\toprule
           Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{n\_blocks} & \texttt{d\_token} & \texttt{d\_main} & \texttt{d\_hidden\_f} & \texttt{d\_drop\_first} & \texttt{d\_drop\_sec.} &                                                 Arch. \\
\midrule
     \texttt{aloi} &            Adam &              $1e-04$ &               $1e-05$ &      \texttt{False} &              &       &                AdamW &                   $1e-05$ &                   &            &                $4$ &             $512$ &            $192$ &                $2.00$ &                  $.15$ &                 $.15$ & \multirow{7}{*}{\rotatebox[origin=c]{-90}{TabResnet}} \\
     \texttt{bank} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-04$ &                   &            &                $3$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
   \texttt{giveme} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-04$ &                   &            &                $4$ &             $448$ &            $448$ &                $1.00$ &                  $.30$ &                 $.40$ &                                                       \\
   \texttt{helena} &            Adam &              $1e-04$ &               $1e-06$ &       \texttt{True} &              &       &                AdamW &                   $1e-07$ &                   &            &                $3$ &             $128$ &            $512$ &                $3.00$ &                  $.25$ &                 $.40$ &                                                       \\
   \texttt{indian} &           AdamW &              $1e-04$ &               $1e-04$ &       \texttt{True} &              &       &                 Adam &                   $1e-05$ &                   &            &                $1$ &             $128$ &            $320$ &                $1.00$ &                  $.35$ &                 $.25$ &                                                       \\
\texttt{miniboone} &            Adam &              $1e-02$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-04$ &                   &            &                $2$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
\texttt{ucicredit} &            Adam &              $1e-02$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-04$ &                   &            &                $2$ &              $64$ &            $128$ &                $2.00$ &                  $.40$ &                 $.45$ &                                                       \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
                Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{zero\_init\_resid} &                                                    Arch. \\
\midrule
         \texttt{MNIST} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} & \multirow{17}{*}{\rotatebox[origin=c]{-90}{Resnet18-50}} \\
    \texttt{bloodmnist} &             SGD &              $1e-01$ &               $1e-04$ &       \texttt{True} &             $.9$ &    \texttt{False} &                 Adam &                   $1e-06$ &                   &            &             \texttt{False} &                                                          \\
   \texttt{breastmnist} &            Adam &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
    \texttt{chestmnist} &             SGD &              $1e-01$ &               $1e-03$ &       \texttt{True} &            $.98$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &             \texttt{False} &                                                          \\
    \texttt{dermamnist} &           AdamW &              $1e-05$ &               $1e-05$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
       \texttt{food101} &             SGD &              $1e-03$ &               $1e-03$ &       \texttt{True} &            $.99$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &             \texttt{False} &                                                          \\
      \texttt{octmnist} &             SGD &              $1e-02$ &               $1e-04$ &       \texttt{True} &            $.95$ &     \texttt{True} &                 Adam &                   $1e-05$ &                   &            &             \texttt{False} &                                                          \\
   \texttt{organamnist} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-04$ &                 $.99$ &          \texttt{True} &             \texttt{False} &                                                          \\
   \texttt{organcmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{organsmnist} &             SGD &              $1e-02$ &               $1e-03$ &       \texttt{True} &            $.96$ &     \texttt{True} &                 Adam &                   $1e-06$ &                   &            &             \texttt{False} &                                                          \\
    \texttt{oxfordpets} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                  SGD &                   $1e-05$ &                 $.97$ &         \texttt{False} &             \texttt{False} &                                                          \\
     \texttt{pathmnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-06$ &                   &            &              \texttt{True} &                                                          \\
\texttt{pneumoniamnist} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                  SGD &                   $1e-06$ &                 $.95$ &          \texttt{True} &             \texttt{False} &                                                          \\
   \texttt{retinamnist} &           AdamW &              $1e-05$ &               $1e-04$ &      \texttt{False} &              &       &                 Adam &                   $1e-07$ &                   &            &             \texttt{False} &                                                          \\
  \texttt{stanfordcars} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &              \texttt{True} &                                                          \\
   \texttt{tissuemnist} &            Adam &              $1e-03$ &               $1e-03$ &       \texttt{True} &              &       &                 Adam &                   $1e-08$ &                   &            &             \texttt{False} &                                                          \\
    \texttt{waterbirds} &            Adam &              $1e-04$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-08$ &                   &            &              \texttt{True} &                                                          \\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccccccccccccc}
\toprule
          Dataset & \texttt{optim.} & \texttt{learn. rate} & \texttt{weight decay} & \texttt{time decay} & \texttt{mom. SGD} & \texttt{nesterov} & \texttt{optim. unc.} & \texttt{learn. rate unc.} & \texttt{mom. SGD unc.} & \texttt{nesterov unc.} & \texttt{b\_norm} &                                           Arch. \\
\midrule
    \texttt{SVHN} &            Adam &              $1e-04$ &               $1e-03$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &    \texttt{True} & \multirow{3}{*}{\rotatebox[origin=c]{-90}{VGG}} \\
\texttt{catsdogs} &           AdamW &              $1e-03$ &               $1e-05$ &      \texttt{False} &              &       &                 Adam &                   $1e-05$ &                   &            &   \texttt{False} &                                                 \\
 \texttt{cifar10} &            Adam &              $1e-03$ &               $1e-04$ &      \texttt{False} &              &       &                AdamW &                   $1e-07$ &                   &            &    \texttt{True} &                                                 \\
\bottomrule
\end{tabular}

 }
 \end{sidewaystable}


==> tex_files/introduction.tex <==
\section{Introduction}
Artificial Intelligence (AI) systems are increasingly being deployed to support or even automate decision-making. In most application scenarios, it is crucial to ensure that the AI systems are trustworthy \citep{DBLP:journals/csur/KaurURD23}, e.g.,  %particularly acute 
in social-sensitive domains such as  healthcare or access to credit.  With reference to Machine Learning (ML) models, a potential way to improve the trustworthiness of a model consists of allowing it to abstain from making a prediction when there is a high risk of making an error \citep{DBLP:journals/tit/Chow70}.
Among the several frameworks for building ML classifiers that can abstain, 
Selective Classification (SC) \citep{DBLP:journals/jmlr/El-YanivW10} aims at trading-off the ratio of abstentions (or, equivalently, the ratio of predictions -- called the \textit{the coverage}) for the predictive performances on the set of instances with a prediction.

The appeal of SC has seen the development of a wide range of approaches for this problem setting \citep{DBLP:conf/nips/GeifmanE17,DBLP:conf/icml/GeifmanE19,DBLP:conf/nips/LiuWLSMU19,DBLP:conf/nips/Huang0020,DBLP:conf/aistats/GangradeKS21,PugnanaRuggieri2023a,PugnanaRuggieri2023b,feng2023towards}, many of which specifically designed for Deep Neural Network (DNN) architectures.
Despite the increasing attention devoted to SC, there is no comprehensive benchmark study of existing methods over a large and diverse collection of dataset and experimental settings. Typical empirical evaluations are limited to partial comparisons over a restricted number of datasets, methods, and performance metrics. All
evaluations have always been conducted on less than ten datasets, never considered more than seven baselines, and they focused mainly on predictive accuracy.
Moreover, given the focus on neural network approaches, prior works primarily experimented with image data only. %, which is not the only setting where SC is useful. 
As a result of the lack of extensive benchmarks, there is a limited understanding of the strengths and weaknesses of the approaches in the literature.


We aim to fill the above gap by presenting a comprehensive evaluation of existing SC methods for DNN architectures. This paper makes the following contributions:

\begin{itemize}
    \item[\textit{(i)}] we briefly survey the state-of-the-art methods in SC, and pose five research questions relevant to evaluate the strengths of such methods and of novel future proposals;
    \item[\textit{(ii)}] we provide the widest experimental evaluation of SC methods in terms of baselines, datasets and tasks;
    \item[\textit{(iii)}] we point out the limitations of compared methods, making the grounds for future research directions;
    \item[\textit{(iv)}] we release a public repository with all software code and datasets for reproducing the baseline algorithms and the experiments\footnote{The code is available at \href{https://github.com/andrepugni/ESC/}{\texttt{github.com/andrepugni/ESC/}}.}.
\end{itemize}
 

==> tex_files/tables/table_data_old.tex <==
\begin{tabular}{cccc}
\toprule
\textbf{Dataset} & \textbf{Data Type} & \textbf{Link} & \textbf{Previous SC paper}\\
\midrule
\texttt{adult} & Tabular & \url{http://archive.ics.uci.edu/dataset/2/adult} & Yes\\
\texttt{aloi} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=1592} & No \\
\texttt{bank} & Tabular & \url{http://archive.ics.uci.edu/dataset/222/bank+marketing} & No\\
\texttt{bloodmnist} & Image & \url{https://zenodo.org/records/6496656/files/bloodmnist.npz?download=1} & No\\
\texttt{breastmnist} & Image & \url{https://zenodo.org/records/6496656/files/breastmnist.npz?download=1} & No \\
\texttt{catsdogs} & Image & \url{https://www.kaggle.com/competitions/dogs-vs-cats/data} & Yes\\
\texttt{chestmnist} & Image & \url{https://zenodo.org/records/6496656/files/chestmnist.npz?download=1} & No \\
\texttt{cifar10} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.CIFAR10.html\#torchvision.datasets.CIFAR10} & Yes\\
\texttt{compass} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44162} & No \\
\texttt{covtype} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=1596} & No \\
\texttt{dermamnist} & Image & \url{https://zenodo.org/records/6496656/files/dermamnist.npz?download=1} & No \\
\texttt{electricity} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44120} & No \\
\texttt{eye} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44157} & No \\
\texttt{food101} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.Food101.html\#torchvision.datasets.Food101} & Yes\\
\texttt{giveme} & Tabular & \url{https://www.kaggle.com/competitions/GiveMeSomeCredit/data?select=cs-training.csv} & Yes \\
\texttt{helena} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=41169} & No\\
\texttt{heloc} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=45023} & No\\
\texttt{higgs} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=23512} & No\\
\texttt{house} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=43957} & No\\
\texttt{indian} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=41972} & No\\
\texttt{jannis} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44079} & No\\
\texttt{kddipums97} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44124} & No \\
\texttt{letter} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=6} & No\\
\texttt{magic} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44125} & No\\
\texttt{miniboone} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44119} & No\\
\texttt{MNIST} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.MNIST.html\#torchvision.datasets.MNIST} & Yes \\
\texttt{octmnist} & Image & \url{https://zenodo.org/records/6496656/files/octmnist.npz?download=1} & No\\
\texttt{online} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=45060} & No\\
\texttt{organamnist} & Image & \url{https://zenodo.org/records/6496656/files/organamnist.npz?download=1} & No \\
\texttt{organcmnist} & Image & \url{https://zenodo.org/records/6496656/files/organcmnist.npz?download=1} & No \\
\texttt{organsmnist} & Image & \url{https://zenodo.org/records/6496656/files/organsmnist.npz?download=1} & No \\
\texttt{oxfordpets} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.OxfordIIITPet.html\#torchvision.datasets.OxfordIIITPet} & No \\

\texttt{pathmnist} & Image & \url{https://zenodo.org/records/6496656/files/pathmnist.npz?download=1} & No \\
\texttt{phoneme} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44127} & No\\

\texttt{pneumoniamnist} & Image & \url{https://zenodo.org/records/6496656/files/pneumoniamnist.npz?download=1} & No \\
\texttt{pol} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=43991} & No\\
\texttt{retinamnist} & Image & \url{https://zenodo.org/records/6496656/files/retinamnist.npz?download=1} & No \\
\texttt{rl} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44160} & No\\
\texttt{stanfordcars} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.StanfordCars.html\#torchvision.datasets.StanfordCars} & Yes\\
\texttt{SVHN} & Image & \url{https://pytorch.org/vision/stable/generated/torchvision.datasets.SVHN.html\#torchvision.datasets.SVHN} & Yes\\
\texttt{tissuemnist} & Image & \url{https://zenodo.org/records/6496656/files/tissuemnist.npz?download=1} & No \\
\texttt{ucicredit} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=42477} & Yes\\
\texttt{upselling} & Tabular & \url{https://www.openml.org/search?type=data\&status=active\&id=44158} & No\\
\texttt{waterbirds} & Image & \url{https://nlp.stanford.edu/data/dro/waterbird\_complete95\_forest2water2.tar.gz} & Yes \\
\bottomrule
\end{tabular}%
